Keypoint Cascade Voting for Point Cloud Based 6DoF Pose Estimation

We propose a novel keypoint voting 6DoF object pose estimation method, which takes pure unordered point cloud geometry as input without RGB information. The proposed cascaded keypoint voting method, called RCVPose3D, is based upon a novel architecture which separates the task of semantic segmentation from that of keypoint regression, thereby increasing the effectiveness of both and improving the ultimate performance. The method also introduces a pairwise constraint in between different keypoints to the loss function when regressing the quantity for keypoint estimation, which is shown to be effective, as well as a novel Voter Confident Score which enhances both the learning and inference stages. Our proposed RCVPose3D achieves state-of-the-art performance on the Occlusion LINEMOD (74.5%) and YCB-Video (96.9%) datasets, outperforming existing pure RGB and RGB-D based methods, as well as being competitive with RGB plus point cloud methods.

==> figs/fig-pipeline.tex <==
\begin{figure*}[h]
\begin{center}
  \includegraphics[width=0.9\textwidth]{figs/rcvpose3d_presem.pdf}
  \caption{The network pipeline.}
  \label{fig:train}
\end{center}
\end{figure*}

==> figs/fig_framework2.tex <==
\begin{figure}[h]
\begin{center}
  \includegraphics[width=0.45\textwidth]{figs/framework2.png}
  \caption{Proposed Cascaded Keypoint Voting Framework: $I$=input image, $E$=encoder-decoder network, $\cal{S}$=segmentation tensor, $\cal{M}$=regression tensor, $V$=voting module, $\cal{K}$=estimated keypoint coordinates, $P$=pose estimation module, $\cal{P}$=output estimated 6DoF object poses}
  \label{fig:framework2}
\end{center}
\end{figure}

==> figs/fig_pipline_box.tex <==
\begin{figure*}[h]
\begin{center}
  \includegraphics[width=0.9\textwidth]{figs/model_rev1.pdf}
  \caption{The network pipeline.}
  \label{fig:train}
\end{center}
\end{figure*}

==> figs/fig_pipline_old.tex <==
\begin{figure*}[h]
\begin{center}
  \includegraphics[width=0.9\textwidth]{figs/rcvpose3d_presem.pdf}
  \caption{The network pipeline.}
  \label{fig:train}
\end{center}
\end{figure*}

==> tabs/YCB-mean-rev1.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{c|c|c|c}\cline{3-4}
\multicolumn{1}{c}{}&\multicolumn{1}{c|}{}&ADD-S&ADD(S)\\\cline{1-2}
  Method  & ICP & AUC & AUC \\\hline\hline
  
     & \xmark  & 75.8 & 59.9\\\cline{2-4}
 \multirow{-2}{*}{PoseCNN~\cite{posecnn} } & \checkmark & 93.0 & 85.4\\\hline
 
& \xmark&94.4 & 82.5\\\cline{2-4}
 \multirow{-2}{*}{BaseNet~\cite{gao20206d} } & \checkmark & - & - \\\hline

 
     & \xmark&91.2& 82.9\\\cline{2-4}
 \multirow{-2}{*}{DF(per-pixel)\cite{wang2019densefusion}} & \checkmark & 93.2&86.1\\\hline

 
     & \xmark&95.5& 91.8\\\cline{2-4}
 \multirow{-2}{*} {PVN3D\cite{pvn3d}}& \checkmark & 96.1& 92.3\\\hline
 
     & \xmark&96.6& 92.7\\\cline{2-4}
 \multirow{-2}{*}{FFB6D\cite{he2021ffb6d}} & \checkmark & -&-\\\hline
 
      & \xmark&96.6&95.2\\\cline{2-4}
 \multirow{-2}{*}{RCVPose~\cite{wu2021vote}} & \checkmark & \textbf{97.2}&\underline{95.9}\\\hline
 
      & \xmark&96.3&95.7\\\cline{2-4}
 \multirow{-2}{*}{Proposed} & \checkmark & \underline{96.6}& \textbf{96.0}\\\hline
\end{tabular}
\caption{YCB Video ADD-S AUC~\cite{posecnn} and ADD(S) AUC results: Non-symmetric objects are evaluated with ADD, and
symmetric objects
(annotated with~$^{*}$) are evaluated with ADD(S) AUC. The ADD-S AUC metrics is based on the curve with ADD-S for all objects. Our ADD(S) AUC surpass the second best RCVPose~\cite{wu2021vote} using RGB by $0.1\%$.
\label{tab:YCBVideoFull}
}
\end{center}
\end{table}


==> tabs/YCB-mean.tex <==
\begin{table}[ht]
\begin{center}
\begin{tabular}{c|c|c|c}
\hline
  Method & Metric & ICP & Mean \\\hline\hline
  
    & ADD-S & \xmark&75.8\\\cline{3-4}
 \multirow{2}{*}{PoseCNN~\cite{posecnn} } &AUC & \checkmark & 93.0\\\cline{2-4}
 &ADD(S) & \xmark & 59.9\\\cline{3-4}
 &AUC & \checkmark & 85.4\\\hline
 
     & ADD-S & \xmark&94.4\\\cline{3-4}
 \multirow{2}{*}{BaseNet~\cite{gao20206d} } &AUC & \checkmark & -\\\cline{2-4}
 &ADD(S) & \xmark & 82.5\\\cline{3-4}
 &AUC & \checkmark & -\\\hline
 
      & ADD-S & \xmark&91.2\\\cline{3-4}
 \multirow{2}{*}{DF(per-pixel)\cite{wang2019densefusion}} &AUC & \checkmark & 93.2\\\cline{2-4}
 &ADD(S) & \xmark & 82.9\\\cline{3-4}
 &AUC & \checkmark & 86.1\\\hline
 
       & ADD-S & \xmark&95.5\\\cline{3-4}
 \multirow{2}{*} {PVN3D\cite{pvn3d}}&AUC & \checkmark & 96.1\\\cline{2-4}
 &ADD(S) & \xmark & 91.8\\\cline{3-4}
 &AUC & \checkmark & 92.3\\\hline
 
       & ADD-S & \xmark&96.6\\\cline{3-4}
 \multirow{2}{*}{FFB6D\cite{he2021ffb6d}} &AUC & \checkmark & -\\\cline{2-4}
 &ADD(S) & \xmark & 92.7\\\cline{3-4}
 &AUC & \checkmark & -\\\hline
 
       & ADD-S & \xmark&96.6\\\cline{3-4}
 \multirow{2}{*}{RCVPose~\cite{wu2021vote}} &AUC & \checkmark & \textbf{97.2}\\\cline{2-4}
 &ADD(S) & \xmark & 95.2\\\cline{3-4}
 &AUC & \checkmark & \underline{95.9}\\\hline
 
        & ADD-S & \xmark&96.3\\\cline{3-4}
 \multirow{2}{*}{Proposed} &AUC & \checkmark & \underline{96.6}\\\cline{2-4}
 &ADD(S) & \xmark & 95.7\\\cline{3-4}
 &AUC & \checkmark & \textbf{96.0}\\\hline
\end{tabular}
\caption{YCB Video ADD-S AUC~\cite{posecnn} and ADD(S) AUC results: Non-symmetric objects are evaluated with ADD, and
symmetric objects
(annotated with~$^{*}$) are evaluated with ADD(S) AUC. The ADD-S AUC metrics is based on the curve with ADD-S for all objects. Our ADD(S) AUC surpass the second best RCVPose~\cite{wu2021vote} using RGB by $0.1\%$.
\label{tab:YCBVideoFull}
}
\end{center}
\end{table}


==> tabs/classified6DWorks-3.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{ccccc}
\cline{1-5}
% \multicolumn{1}{c}{} &
\multicolumn{1}{c}{\multirow{2}{*}{Method} } &
% \multirow{2}{c}{Method} &
\multicolumn{1}{c}{Publication} &\multicolumn{3}{c}{Data Mode} \\
%\cline{1-1}
% Method 
& Date & RGB & D & 3D \\
\hline \hline
Tekin et al. \cite{yolo6d} & 2017 & \checkmark & & \\  
SSD-6D \cite{kehl2017ssd}& 2017  & \checkmark &  & \\
Pix2Pose \cite{park2019pix2pose} & 2019 & \checkmark & &  \\ 
DPOD \cite{zakharov2019dpod}& 2019 & \checkmark &  &  \\ 
Trabelsi et al. \cite{trabelsi2021ppn}& 2021 & \checkmark & &  \\ 
Dsc-posenet \cite{yang2021dsc} & 2021 & \checkmark & & \\ 
GDR-Net \cite{wang2021gdr}& 2021 & \checkmark &  & \\
\hline

PoseCNN \cite{posecnn}& 2017 & \checkmark & \checkmark & \\ 
Tian et al. \cite{tian2020robust}&2020& \checkmark & \checkmark  &\\

StablePose \cite{shi2021stablepose}& 2021 & \checkmark & \checkmark & \\  
SO-Pose \cite{Di_2021_ICCV}&2021& \checkmark & \checkmark  &\\
\hline

PVN3D \cite{pvn3d} & 2019 & \checkmark & & \checkmark \\
DenseFusion \cite{wang2019densefusion}& 2019 & \checkmark & & \checkmark \\ 
PointVoteNet \cite{hagelskjaer2020pointvotenet}& 2020 & \checkmark & & \checkmark \\ 
FFB6D \cite{he2021ffb6d}& 2021 & \checkmark & & \checkmark \\\hline

RCVPose \cite{wu2021vote}& 2021 & \checkmark & \checkmark & \checkmark \\ \hline
OP-Net~\cite{OPNet} & 2019 & & \checkmark &  \\\hline
BaseNet~\cite{gao20206d} & 2020 & & & \checkmark \\
RCVPose3D& 2022 & & & \checkmark \\ \hline
% \\ \hline
\end{tabular}
\end{center}
\vspace{-1\baselineskip}
\caption{Methods with various input data modes}
\vspace{-1\baselineskip}
\label{tab:MethodsWithDiffInput}
\end{table}

==> tabs/classified6DWorks.tex <==
\begin{table}[]
\begin{center}
\begin{tabular}{|c|c|}
\hline
Input data                & Method                           \\ \hline
\multirow{4}{*}{pure RGB} & Pix2Pose \cite{park2019pix2pose} \\ \cline{2-2} 
                          & Tekin et al. \cite{yolo6d}                               \\ \cline{2-2} 
                          & Trabelsi et al. \cite{trabelsi2021ppn}                               \\ \cline{2-2} 
                          & Dsc-posenet \cite{yang2021dsc}                                \\ \hline
\multirow{4}{*}{RGB with ICP}  &   DPOD \cite{zakharov2019dpod}                                   \\ \cline{2-2}
                          &   SSD-6D \cite{kehl2017ssd}                               \\ \cline{2-2}
                          &   PoseCNN \cite{posecnn}                               \\ \cline{2-2}
                          & GDR-Net \cite{wang2021gdr} \\ \hline
\multirow{3}{*}{RGB with Depth} & RCVPose \cite{wu2021vote}                             \\ \cline{2-2}
                          & StablePose \cite{shi2021stablepose} \\ \cline{2-2}
                          & PointVoteNet \cite{hagelskjaer2020pointvotenet} \\ \hline
\multirow{3}{*}{RGB with Point Cloud}      &   PVN3D \cite{PVN3d}                               \\ \cline{2-2}
                          &  FFB6D \cite{he2021ffb6d} \\ \cline{2-2}
                          &  DenseFusion \cite{wang2019densefusion}                              \\ \hline
\end{tabular}
\end{center}
\caption{Methods with different input}
\label{tab:MethodsWithDiffInput}
\end{table}

==> tabs/e2evs2s.tex <==

\begin{table}[ht]
\begin{center}
\begin{tabular}{l|c|c|c|c}
\hline
\multicolumn{2}{c|}{Framework}&Parallel&Parallel&Cascade\\\hline
\multicolumn{2}{c|}{Loss Function}&$\mathcal{L}_{\epsilon}\!+\!\mathcal{L}_{P}$, $\mathcal{L}_{bce}\!+\!\mathcal{L}_{P}$, $\mathcal{L}_{bce}$\\\hline
 %Stage & Metric & 1S($\mathcal{L}_{sl1}$) & 1S($\mathcal{L}_{geo}$ \& $\mathcal{L}_{bce}$) & 2S \\\hline
& mIOU &  85.6 & 91.2 &  100    \\
training    & VCS &  53.2 & 61.2 &  95.2      \\
       & ADD(s) &  75.2 & 84.2 &  100          \\\hline
  & mIOU &  63.2 & 76.3 &  \textbf{91.7}\\
testing    & VCS &  49.7 & 58.3 &  \textbf{91.1}         \\
    & ADD(s) &  40.2 & 50.4 &  \textbf{65.7}         \\\hline
\end{tabular}
\end{center}
\caption{Parallel vs Cascade: The semantic segmentation benefits from the Cascade framework with a better mIOU initially. The VCS of Cascade framework is also $42\%$ / $34\%$ better than both parallel frameworks with different losses when being trained on the object of ape and $41.4\%$ / $32.8\%$ better when testing on ape in LMO. The ADD(s) also matches the VCS result and proposed 2S framework works the best among all three tested. }
\label{tab:e2evs2s}
\end{table}

==> tabs/e2evs2s_adds.tex <==

\begin{table}[ht]
\begin{center}
\begin{tabular}{l|c|c|c|c}
\hline
\multicolumn{2}{c|}{Architecture}&Parallel&Parallel&Cascade\\\hline
\multicolumn{2}{c|}{Loss Function}&$\mathcal{L}_{\epsilon}$&$\mathcal{L}_{P}$, $\mathcal{L}_{bce}$&$\mathcal{L}_{P}$, $\mathcal{L}_{bce}$\\\hline
\multirow{2}{*}{ADD(S)}    & training &  75.2 & 84.2 &  100          \\\cline{2-5}
& testing &  40.2 & 50.4 &  \textbf{65.7}         \\\hline
\end{tabular}
\end{center}
\caption{ADD(S) of Parallel vs Cascade: The ADD(S) matches the VCS result and proposed Cascade framework works the best among all three architectures tested. }
\label{tab:e2evs2sadds}
\end{table}

==> tabs/e2evs2s_miou.tex <==

% \begin{table}[ht]
% \begin{center}
% \begin{tabular}{l|c|c|c|c}
% \hline
% \multicolumn{2}{c|}{Architecture}&\multicolumn{2}{c|}{Parallel}&Cascade\\\hline
% \multicolumn{2}{c|}{Loss Function}&$\mathcal{L}_{sl1}$&$\mathcal{L}_{r}\!+\!\mathcal{L}_{bce}$&$\mathcal{L}_{r}\!+\!\mathcal{L}_{bce}$\\\hline
%  %Stage & Metric & 1S($\mathcal{L}_{sl1}$) & 1S($\mathcal{L}_{geo}$ \& $\mathcal{L}_{bce}$) & 2S \\\hline
% \multirow{2}{*}{mIoU}& training &  85.6 & 91.2 &  100    \\
%   \cline{2-5}
%   & testing &  63.2 & 76.3 &  \textbf{91.7}\\\hline
% \end{tabular}
% \end{center}
% \vspace{-1\baselineskip}
% \caption{Parallel vs. Cascade Impact on Semantic Segmentation: The semantic segmentation benefits from the Cascade architecture with a better mIoU on LMO.}
% \label{tab:e2evs2smiou}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[ht]
% \begin{center}
% %   \resizebox{\columnwidth}{!}{%
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{c|c|c|c}
% \cline{3-4}
% \multicolumn{2}{c|}{}&\multicolumn{2}{c}{mIoU}\\\hline
% Architecture   & Loss  & training &testing
% \\\hline \hline
% \multirow{2}{*}{Parallel}
% & $\mathcal{L}_{sl1}$ & 85.6&63.2\\\cline{2-4}
% &\multirow{2}{*}{$\mathcal{L}_{r}\!+\!\mathcal{L}_{bce}$} & 91.2 &\underline{76.3}\\\cline{1-1}\cline{3-4}
% Cascade & &100&\textbf{91.7}\\\hline
% \end{tabular}
% \end{adjustbox}
% \end{center}
% \vspace{-1\baselineskip}
% %   } % \resizebox
% \caption{Performance of Semantic Segmentation in Parallel vs. Cascade architecture.} %The semantic segmentation benefits from the Cascade architecture with a better mIoU on LMO.}
%  \label{tab:e2evs2smiou}
%  \vspace{-1\baselineskip}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\begin{center}
%   \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|c}
\cline{2-3}
\multicolumn{1}{c|}{}
& \multicolumn{2}{c|}{mIoU}\\\hline
Architecture   & training & testing & Loss
\\ \hline \hline
\multirow{2}{*}{Parallel} 
& 85.6 & 63.2 
& $\mathcal{L}_{s}$\\\cline{2-4}
 & 91.2 &\underline{76.3}
 & $\mathcal{L}_{r}\!+\!\mathcal{L}_{bce}$\\
 \cline{1-4}
Cascade & 100 & \textbf{91.7}& $\mathcal{L}_{r}$, $\mathcal{L}_{bce}$
\\\hline

\end{tabular}
\end{adjustbox}
\end{center}
\vspace{-1\baselineskip}
%   } % \resizebox
\caption{Performance (mIoU) of segmentation  for parallel vs. cascade architectures and varying losses, on LMO} %The semantic segmentation benefits from the Cascade architecture with a better mIoU on LMO.}
 \label{tab:e2evs2smiou}
 \vspace{-1\baselineskip}
\end{table}

==> tabs/e2evs2s_occLINEMODFull.tex <==
% \begin{comment}
% \begin{table*}[h]
% %   \resizebox{\columnwidth}{!}{%
% %   \resizebox{\pagewidth}{!}{%
% \begin{center}
% %   \begin{tabularx}
% \vspace{1.25 cm} \\
% \begin{tabular}
% {r|c|c|c|c|c|c|c|c|c|c|c|c|c}
% %   \cline{1-1} \\
% \multicolumn{1}{c|}{Object}      &
% %   Object &
% \begin{rotate}{60} 
% YOLO6D 
% \end{rotate} & 
% \begin{rotate}{60} 
% SSD6D+ref 
% \end{rotate}
% & 
% \begin{rotate}{60} 
% PoseCNN 
% \end{rotate}
% & 
% \begin{rotate}{60} 
% Oberweger 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  Hu et al. 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  Pix2Pose
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  DPOD
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PVNet
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  DPOD+ref 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PPRN 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PVN3D 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PoseCNN+ICP 
% \end{rotate}
% &  
% \begin{rotate}{60} 
%  RCVPose
% \end{rotate}
% \\ \hline \hline
% ape         & -                                 & -                                    & 9.6                                  & 12.1                                   & 17.6                                   & 22                                    & -                               & 15.8                              & -                    & -              & 33.9                               & 76.2                & 60.3 \\ \hline
% can         & -                                 & -                                    & 45.2                                 & 39.9                                   & 53.9                                   & 44.7                                  & -                               & 63.3                               & -                    & -               & 88.6                               & 87.4               & 92.5  \\ \hline
% cat         & -                                 & -                                    & 0.93                                 & 8.2                                    & 3.3                                    & 22.7                                  & -                               & 16.7                             & -                    & -                & 39.1                               & 52.2              & 50.2   \\ \hline
% driller     & -                                 & -                                    & 41.4                                 & 45.2                                   & 62.4                                   & 44.7                                  & -                               & 25.2                            & -                    & -                & 78.4                               & 90.3              &78.2   \\ \hline
% duck        & -                                 & -                                    & 19.6                                 & 17.2                                   & 19.2                                   & 15                                    & -                               & 65.6                            & -                    & -                 & 41.9                               & 77.7             & 52.1   \\ \hline
% eggbox      & -                                 & -                                    & 22                                   & 22.1                                   & 25.9                                   & 25.2                                  & -                               & 50.2                              & -                    & -                 & 80.9                               & 72.2             & 81.2    \\ \hline
% glue        & -                                 & -                                    & 38.5                                 & 35.8                                   & 39.6                                   & 32.4                                  & -                               & 49.6                              & -                    & -                & 68.1                               & 76.7              & 72.0   \\ \hline
% holepuncher & -                                 & -                                    & 22.1                                 & 36                                     & 21.3                                   & 49.5                                  & -                               & 39.7                              & -                    & -                 & 74.7                               & 91.4             & 75.2   \\ \hline \hline
% mean        & 6.4                               & 27.5                                   & 24.9                                 & 27                                     & 27                                     & 32                                    & 32.8                             & 40.8                              & 47.2                 & 58.4              & 63.2                               & 78               & 70.2    \\ \hline
% %   \end{tabularx}
% \end{tabular}
% \end{center}
% \\
% \caption{Occlusion LINEMOD Leaderboard}
% \label{tab:OccLinemod}
% %   } % \resizebox
% \end{table*}
% \end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\begin{center}
%   \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
\cline{4-12}
\multicolumn{3}{c|}{}
&
\multicolumn{7}{c}{Object} & \multirow{2}{*}{hole-}  
& $\overline{\mbox{ADD(s)}}$ \\ % [3pt]
\cline{1-3}
%   \cline{11-11}
%   \hline
framework   & Loss  & ICP     & ape  & can  & cat  & driller & duck & eggbox$^{*}$ & glue$^{*}$ & puncher &
% \begin{tabular}{c}\vspace{-3 pt} 
% $\overline{\mbox{ADD(s)}} [\%]$ 
% \end{tabular}
$ [\%]$
\\\hline \hline

& \multirow{1}{*}{$\mathcal{L}_{\epsilon}$} & \xmark & 39.8 & 67.4 & 32.4 & 67.2  & 20.3 & 65.1  & 45.5 & 61.3 & 49.9 \\ \cline{3-12}
&                             & \checkmark & 40.2 & 67.7 & 32.7 & 67.7  & 20.7 & 65.4  & 45.9 & 61.7 & 50.3 \\ \cline{2-12}
\multirow{-1.5}{*}{E2E}
&                                 & \xmark & 49.7 & 78.2 & 45.2 & 75.2  & 42.1 & 71.9  & 57.1 & 72.2 & 61.5 \\ \cline{3-12}
& Binary Cross Entropy Loss & \checkmark   & 50.4 & 78.6 & 45.7 & 75.6  & 42.5 & 72.3  & 57.4 & 72.6 & 61.9 \\ \cline{1-1}\cline{3-12}
\multirow{-0.5}{*}{2S}
& + Geo Constraint Loss & \xmark           & 63   & 96.1 & 57.3 & 81.4  & 54.2 & 81.5  & 75.1 & 80.7 & 73.7\\ \cline{3-12}
&  & \checkmark                            & \textbf{65.7} & \textbf{96.4} & \textbf{58.5} & \textbf{81.7}  & \textbf{54.7} & \textbf{82}    & \textbf{75.4} & \textbf{81.2} & \textbf{74.5}\\ \hline

\end{tabular}
\end{adjustbox}
\end{center}
%   } % \resizebox
\caption{LMO Accuracy Results with different strctures.
Non-symmetric objects are evaluated with ADD, and
symmetric objects
(annotated with~$^{*}$) are evaluated with ADD-s. The 2S framework with Radial Pair Loss and Binary Cross Entropy Loss is apparently better than any other configurations.
\label{tab:e2evs2sfull}\vspace{+10pt}
}
\end{table*}

==> tabs/e2evs2s_vcs.tex <==

% \begin{table}[ht]
% \begin{center}
% \begin{tabular}{c|c|c|c}
% \cline{3-4}
% \multicolumn{2}{c|}{}&\multicolumn{2}{c}{VCS}\\\hline
% Architecture   & Loss  & training &testing
% \\\hline \hline
% \multirow{2}{*}{Parallel}
% & $\mathcal{L}_{sl1}$ & 54.5&52.1\\\cline{2-4}
% &\multirow{2}{*}{$\mathcal{L}_{r}\!+\!\mathcal{L}_{bce}$} & 63.5&\underline{61.7}\\\cline{1-1}\cline{3-4}
% Cascade & &95.4  &\textbf{93.7} \\\hline
% % \begin{tabular}{l|c|c|c|c}
% % \hline
% % \multicolumn{2}{c|}{Architecture}&\multicolumn{2}{c|}{Parallel}&Cascade\\\hline
% % \multicolumn{2}{c|}{Loss Function}&$\mathcal{L}_{sl1}$ & $\mathcal{L}_{r}\!+\! \mathcal{L}_{bce}$ & $\mathcal{L}_{r}\!+\!\mathcal{L}_{bce}$\\\hline
% % \multirow{2}{*}{VCS}    & training &  54.5 & \underline{63.5} &  \textbf{95.4}      \\\cline{2-5}
%     % & testing &  52.1 & \underline{61.7} &  \textbf{93.7}         \\\hline
% \end{tabular}
% \end{center}
% \vspace{-1\baselineskip}
% \caption{Performance (VCS) of Regression for Parallel vs. Cascade Architectures and Varying Losses.} %The VCS of Cascade architecture is also $42\%$ / $34\%$ better than both parallel architecture with different losses during training and $41.4\%$ / $32.8\%$ better during testing on LMO.}
% \label{tab:e2evs2svcs}
% \vspace{-1\baselineskip}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[t]
\begin{center}
%   \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|c}
\cline{2-3}
\multicolumn{1}{c|}{}
& \multicolumn{2}{c|}{VCS}\\\hline
Architecture   & training & testing & Loss
\\ \hline \hline
\multirow{2}{*}{Parallel} 
& 54.5 & 52.1 
& $\mathcal{L}_{s}$\\\cline{2-4}
 & 63.5 &\underline{61.7}
 & $\mathcal{L}_{r}\!+\!\mathcal{L}_{bce}$\\
 \cline{1-4}
Cascade & 95.4 & \textbf{93.7}& $\mathcal{L}_{r}$, $\mathcal{L}_{bce}$
\\\hline

\end{tabular}
\end{adjustbox}
\end{center}
\vspace{-1\baselineskip}
%   } % \resizebox
\caption{Performance (VCS) of regression for parallel vs. cascade architectures and varying losses, on LMO} %The semantic segmentation benefits from the Cascade architecture with a better mIoU on LMO.}
 \label{tab:e2evs2svcs}
 \vspace{-0.7\baselineskip}
\end{table}

==> tabs/kMeansVoting.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\begin{center}
\resizebox{.9\columnwidth}{!}{%
\begin{tabular}{r|c|cc|cc|cc}
\cline{3-8}
\multicolumn{2}{c}{} &
\multicolumn{6}{c}{$\bar{\epsilon}$ [mm]} \\
 %  \cline{3-8}
\multicolumn{2}{l}{} & \multicolumn{2}{c}{vector}                & \multicolumn{2}{c}{offset}                    & \multicolumn{2}{c}{ radial}               \\[-5pt]
\cline{2-2} 
 \multicolumn{1}{c}{}
 &
 \multicolumn{1}{c|}{$\bar{r}$ [mm]}
&
\multicolumn{1}{c}{$\mu_v$} & \multicolumn{1}{c}{$\sigma_v$} & \multicolumn{1}{|c}{$\mu_o$} & \multicolumn{1}{c|}{$\sigma_o$} & \multicolumn{1}{c}{$\mu_r$} & \multicolumn{1}{c}{$\sigma_r$} \\ \hline \hline
ape & 61.2 & 10.0 & 5.8 & 5.8 & 2.6 & {\bf 1.3} & {\bf 0.7} \\ \hline
driller & 129.4 & 10.0 & 2.3 & 6.5 & 4.7 & {\bf 2.2} & {\bf 1.0} \\ \hline
eggbox & 82.5 & 11.8 & 5.3 & 5.2 & 2.7 & {\bf 2.0} & {\bf 0.7}\\ 
 \hline
\end{tabular}
} 
\end{center}
\caption{Surface keypoint estimation error:  $\bar{\epsilon}$ mean ($\mu_{\{v|o|r\}}$)  and standard deviation ($\sigma_{\{v|o|r\}}$)
for 3 voting schemes,
with 
$\bar{r}$
= mean distance of keypoints to object centroid.}
\label{tab:KEE-FPS}
\vspace{-1\baselineskip}
\end{table}

==> tabs/occLINEMOD-mean.tex <==
\begin{table}[ht]
\begin{center}
%  \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|c|c}
\cline{3-5}
\multicolumn{2}{c|}{}

& LMO & \multicolumn{2}{c|}{YCB} \\ \cline{3-5}
\multicolumn{2}{c|}{}

& $\overline{\mbox{ADD(s)}}$ & ADD-S &ADD(S \\ 
\cline{1-2}

Mode      & Method & $ [\%]$ &AUC &AUC
\\\hline \hline
                                & Oberweger~\cite{oberweger2018making}   & 27.1 \\\cline{2-3} 
                                & Hu et al.~\cite{hu2019segmentation}   & 30.4 \\\cline{2-3} 
                                & Pix2Pose~\cite{park2019pix2pose}     & 32.0 \\\cline{2-3} 
                                & DPOD~\cite{zakharov2019dpod}   & 32.8 \\\cline{2-3} 
                                & PVNet~\cite{pvnet}       & 40.8 \\\cline{2-3} 
%   \begin{rotate}{90} 
\multirow{-6}{*}{RGB}
%   \end{rotate}
                                & PPRN~\cite{trabelsi2021ppn}    & 58.4 \\\hline\hline
                                & YOLO6D~\cite{yolo6d}    & 6.4  \\\cline{2-3} 
                                & SSD6D+ref~\cite{kehl2017ssd} & 27.5 \\\cline{2-3} 
                               
\multirow{-3}{*}{RGB}      
                                &  PoseCNN~\cite{posecnn}     & 24.9 \\\cline{2-3} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{+D ref}
%   \end{rotate}     
                                & DPOD+ref~\cite{zakharov2019dpod}   & 47.3 \\\hline\hline

                                & RCVPose          & 70.2 \\\cline{2-3} 
%   \begin{rotate}{90} 
\multirow{+2.5}{*}{RGB-D/}  
%   \end{rotate}

& RCVPose+ICP & 71.1\\ \cline{2-3} 
\multirow{+2.5}{*}{RGB+3D}  & PVN3D~\cite{pvn3d}  & 63.2 \\\cline{2-3} 
& FFB6D~\cite{he2021ffb6d}  & 66.2 \\\cline{2-3} 
& PointVoteNet+ICP\cite{hagelskjaer2020pointvotenet}   & \textbf{75.1} \\\hline\hline
\multirow{2}{*}{3D/Mesh}
& Proposed  & 73.7\\ \cline{2-3}
& Proposed + ICP & \underline{74.5}\\ \hline

\end{tabular}
\end{adjustbox}
\end{center}
%  } % \resizebox
\caption{Occlusion LINEMOD Accuracy Results.
Non-symmetric objects are evaluated with ADD, and
symmetric objects
(annotated with~$^{*}$) are evaluated with ADD-s. Proposed method achieves competitive results(underlined) with an ICP refinement compared to methods using RGB.
\label{tab:OccLinemod}
}
\end{table}

==> tabs/occLINEMOD.tex <==
% \begin{comment}
% \begin{table*}[h]
% %   \resizebox{\columnwidth}{!}{%
% %   \resizebox{\pagewidth}{!}{%
% \begin{center}
% %   \begin{tabularx}
% \vspace{1.25 cm} \\
% \begin{tabular}
% {r|c|c|c|c|c|c|c|c|c|c|c|c|c}
% %   \cline{1-1} \\
% \multicolumn{1}{c|}{Object}      &
% %   Object &
% \begin{rotate}{60} 
% YOLO6D 
% \end{rotate} & 
% \begin{rotate}{60} 
% SSD6D+ref 
% \end{rotate}
% & 
% \begin{rotate}{60} 
% PoseCNN 
% \end{rotate}
% & 
% \begin{rotate}{60} 
% Oberweger 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  Hu et al. 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  Pix2Pose
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  DPOD
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PVNet
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  DPOD+ref 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PPRN 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PVN3D 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PoseCNN+ICP 
% \end{rotate}
% &  
% \begin{rotate}{60} 
%  RCVPose
% \end{rotate}
% \\ \hline \hline
% ape         & -                                 & -                                    & 9.6                                  & 12.1                                   & 17.6                                   & 22                                    & -                               & 15.8                              & -                    & -              & 33.9                               & 76.2                & 60.3 \\ \hline
% can         & -                                 & -                                    & 45.2                                 & 39.9                                   & 53.9                                   & 44.7                                  & -                               & 63.3                               & -                    & -               & 88.6                               & 87.4               & 92.5  \\ \hline
% cat         & -                                 & -                                    & 0.93                                 & 8.2                                    & 3.3                                    & 22.7                                  & -                               & 16.7                             & -                    & -                & 39.1                               & 52.2              & 50.2   \\ \hline
% driller     & -                                 & -                                    & 41.4                                 & 45.2                                   & 62.4                                   & 44.7                                  & -                               & 25.2                            & -                    & -                & 78.4                               & 90.3              &78.2   \\ \hline
% duck        & -                                 & -                                    & 19.6                                 & 17.2                                   & 19.2                                   & 15                                    & -                               & 65.6                            & -                    & -                 & 41.9                               & 77.7             & 52.1   \\ \hline
% eggbox      & -                                 & -                                    & 22                                   & 22.1                                   & 25.9                                   & 25.2                                  & -                               & 50.2                              & -                    & -                 & 80.9                               & 72.2             & 81.2    \\ \hline
% glue        & -                                 & -                                    & 38.5                                 & 35.8                                   & 39.6                                   & 32.4                                  & -                               & 49.6                              & -                    & -                & 68.1                               & 76.7              & 72.0   \\ \hline
% holepuncher & -                                 & -                                    & 22.1                                 & 36                                     & 21.3                                   & 49.5                                  & -                               & 39.7                              & -                    & -                 & 74.7                               & 91.4             & 75.2   \\ \hline \hline
% mean        & 6.4                               & 27.5                                   & 24.9                                 & 27                                     & 27                                     & 32                                    & 32.8                             & 40.8                              & 47.2                 & 58.4              & 63.2                               & 78               & 70.2    \\ \hline
% %   \end{tabularx}
% \end{tabular}
% \end{center}
% \\
% \caption{Occlusion LINEMOD Leaderboard}
% \label{tab:OccLinemod}
% %   } % \resizebox
% \end{table*}
% \end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\begin{center}
%   \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\cline{3-11}
\multicolumn{2}{c|}{}
&
\multicolumn{7}{c}{Object} & \multirow{2}{*}{hole-}  
\\%& %$\overline{\mbox{ADD(s)}}$ \\ % [3pt]
\cline{1-2}
%   \cline{11-11}
%   \hline
Mode      & Method     & ape  & can  & cat  & driller & duck & eggbox$^{*}$ & glue$^{*}$ & puncher &
% \begin{tabular}{c}\vspace{-3 pt} 
% $\overline{\mbox{ADD(s)}} [\%]$ 
% \end{tabular}
Mean
%$ [\%]$
\\\hline \hline
                                & Oberweger~\cite{oberweger2018making}  & 12.1 & 39.9 & 8.2  & 45.2    & 17.2 & 22.1   & 35.8 & 36.0        & 27.1 \\\cline{2-11} 
                                & Hu et al.~\cite{hu2019segmentation}  & 17.6 & 53.9 & 3.3  & 62.4    & 19.2 & 25.9   & 39.6 & 21.3        & 30.4 \\\cline{2-11} 
                                & Pix2Pose~\cite{park2019pix2pose}   & 22.0 & 44.7 & 22.7 & 44.7    & 15.0 & 25.2   & 32.4 & 49.5        & 32.0 \\\cline{2-11} 
                                & DPOD~\cite{zakharov2019dpod}       & -  & -  & -  & -     & -  & -    & -  & -         & 32.8 \\\cline{2-11} 
                                & PVNet~\cite{pvnet}      & 15.8 & 63.3 & 16.7 & 25.2    & 65.7 & 50.2   & 49.6 & 39.7        & 40.8 \\\cline{2-11} 
%   \begin{rotate}{90} 
\multirow{-6}{*}{RGB}
%   \end{rotate}
& PPRN~\cite{trabelsi2021ppn}       & -  & -  & -  & -     & -  & -    & -  & -         & 58.4 \\\hline\hline
                                & YOLO6D~\cite{yolo6d}     & -  & -  & -  & -     & -  & -    & -  & -         & 6.4  \\\cline{2-11} 
                                & SSD6D+ref~\cite{kehl2017ssd}  & -  & -  & -  & -     & -  & -    & -  & -         & 27.5 \\\cline{2-11} 
                               
\multirow{-3}{*}{RGB}      
&  PoseCNN~\cite{posecnn}    & 9.6  & 45.2 & 0.9  & 41.4    & 19.6 & 22.0   & 38.5 & 22.1        & 24.9 \\\cline{2-11} 
%   \begin{rotate}{90} 
\multirow{-3}{*}{+D ref}
%   \end{rotate}     
& DPOD+ref~\cite{zakharov2019dpod}   & -  & -  & -  & -     & -  & -    & -  & -         & 47.3 \\\hline\hline

                                & RCVPose     & 60.3 & 92.5 & 50.2 & 78.2    & 52.1 & 81.2   & 72.1  & 75.2        & 70.2 \\\cline{2-11} 
%   \begin{rotate}{90} 
\multirow{+3}{*}{RGB-D/RGB+3D}  
%   \end{rotate}

& RCVPose+ICP & 61.3 & 93 & 51.2 & 78.8  & 53.4 & \textbf{82.3}  & \underline{72.9} & 75.8 & 71.1\\ \cline{2-11} 
& PVN3D~\cite{pvn3d}      & 33.9 & 88.6 & 39.1 & 78.4   & 41.9 & 80.9   & 68.1 & 74.7        & 63.2 \\\cline{2-11} 
& FFB6D~\cite{he2021ffb6d}      & - & - & - & - & - & -   & - & -   & 66.2 \\\cline{2-11} 
& PointVoteNet+ICP\cite{hagelskjaer2020pointvotenet}   & \textbf{70.0} & \underline{95.5} & \textbf{60.8} & \textbf{87.9}   & \textbf{70.7} & 58.7   & 66.9 & \textbf{90.6}        & \textbf{75.1} \\\hline\hline
%   \end{rotate}
% & Radii with Pointnet++(E2E with vanilla smotth l1) & 39.8 & 67.4 & 32.4 & 67.2  & 20.3 & 65.1  & 45.5 & 61.3 & 49.9 \\ \cline{2-11}
% & Radii with Pointnet++(E2E with vanilla smooth l1) + ICP & 40.2 & 67.7 & 32.7 & 67.7  & 20.7 & 65.4  & 45.9 & 61.7 & 50.3 \\ \cline{2-11}
% & Radii with Pointnet++(E2E with geo \& bce) & 49.7 & 78.2 & 45.2 & 75.2  & 42.1 & 71.9  & 57.1 & 72.2 & 61.5 \\ \cline{2-11}
% & Radii with Pointnet++(E2E with geo \& bce) + ICP & 50.4 & 78.6 & 45.7 & 75.6  & 42.5 & 72.3  & 57.4 & 72.6 & 61.9 \\ \cline{2-11}
\multirow{2}{*}{3D/Mesh}
& RCVPose3D & 63   & 96.1 & 57.3 & 81.4  & 54.2 & 81.5  & 75.1 & 80.7 & 73.7\\ \cline{2-11}
& RCVPose3D + ICP & \underline{65.7} & \textbf{96.4} & \underline{58.5} & \underline{81.7}  & \underline{54.7} & \underline{82}    & \textbf{75.4} & \underline{81.2} & \underline{74.5}\\ \hline

% & Radii with Point Transformer & 59.2 & 93.4 & 56.8 & 80.8 & 58.2 & 79.6 & 73.2 & 85.4 & 73.3 \\ \cline{2-11}
% & Radii with Point Transformer + ICP & 59.9  & 93.7 & 57.2 & 81.1 & 58.6 & 80.1 & 73.6 & 85.8 & 73.8 \\ \cline{2-11}
% & Radii with PPF+knn & 55.7 & 88.6 & 51.2 &  78.2 & 54.1 & 79.4  & 73.8 & 85.7 & 70.8 \\\cline{2-11}
% & Radii with PPF+knn + ICP & 56.8 & 89.4 & 51.6 & 78.8 & 54.8 & 80.2  & 74.3 & 87.2 & 71.7 \\\cline{2-11}
% & Radii with FPFH+knn & 55.4 & 89.2 & 50.2 & 77.8 & 52.6 & 80.9  & 72.4 & 86.3 & 70.6 \\\cline{2-11}
% & Radii with FPFH+knn + ICP & 55.7 & 90.2 & 50.8 & 78.2  & 53.8 & 81.4 & 73.2 & 87.2 & 71.3 \\\cline{2-11}
% & Radii with DGCNN\cite{wang2019dgcnn} & 58 & 87.2 & 53.4 & 77.8  & 51.9 & 78.7  & 71.2 & 82.3 & 70.1\\\cline{2-11}
% & Radii with DGCNN+ICP & 59.2 & 88.6 & 54.1 & 78.2  & 52.1 & 78.7  & 71.7 & 82.7 & 70.7 \\\cline{2-11}
% & Radii with subdivnet\cite{hu2021subdivnet} & 42.3 & 83.2 & 49.2 &  77.8 & 48.7 & 77.9  & 69.2 & 75.2 & 65.4\\\cline{2-11}
% & Radii with subdivnet + ICP & 45.2 & 83.7 & 49.7 & 78.2  & 49.2 & 78.2  & 70.1 & 75.2 & 66.2\\\hline

\end{tabular}
\end{adjustbox}
\end{center}
%   } % \resizebox
\caption{LMO accuracy results:
accuracy of 6DoF PE methods for non-symmetric objects are evaluated with ADD, and that of 
symmetric objects
(annotated with~$^{*}$) are evaluated with ADD-s. %Proposed method achieves competitive results with an ICP refinement compared to methods using RGB, specifically for colorless objects like \emph{eggbox} and \emph{can}, the performance outperformed most of the methods including RGB.
\label{tab:OccLinemod}
}
\vspace{2\baselineskip}
\end{table*}

==> tabs/occlinemod_descriptors.tex <==
% \begin{comment}
% \begin{table*}[h]
% %   \resizebox{\columnwidth}{!}{%
% %   \resizebox{\pagewidth}{!}{%
% \begin{center}
% %   \begin{tabularx}
% \vspace{1.25 cm} \\
% \begin{tabular}
% {r|c|c|c|c|c|c|c|c|c|c|c|c|c}
% %   \cline{1-1} \\
% \multicolumn{1}{c|}{Object}      &
% %   Object &
% \begin{rotate}{60} 
% YOLO6D 
% \end{rotate} & 
% \begin{rotate}{60} 
% SSD6D+ref 
% \end{rotate}
% & 
% \begin{rotate}{60} 
% PoseCNN 
% \end{rotate}
% & 
% \begin{rotate}{60} 
% Oberweger 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  Hu et al. 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  Pix2Pose
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  DPOD
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PVNet
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  DPOD+ref 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PPRN 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PVN3D 
% \end{rotate}
% & 
% \begin{rotate}{60} 
%  PoseCNN+ICP 
% \end{rotate}
% &  
% \begin{rotate}{60} 
%  RCVPose
% \end{rotate}
% \\ \hline \hline
% ape         & -                                 & -                                    & 9.6                                  & 12.1                                   & 17.6                                   & 22                                    & -                               & 15.8                              & -                    & -              & 33.9                               & 76.2                & 60.3 \\ \hline
% can         & -                                 & -                                    & 45.2                                 & 39.9                                   & 53.9                                   & 44.7                                  & -                               & 63.3                               & -                    & -               & 88.6                               & 87.4               & 92.5  \\ \hline
% cat         & -                                 & -                                    & 0.93                                 & 8.2                                    & 3.3                                    & 22.7                                  & -                               & 16.7                             & -                    & -                & 39.1                               & 52.2              & 50.2   \\ \hline
% driller     & -                                 & -                                    & 41.4                                 & 45.2                                   & 62.4                                   & 44.7                                  & -                               & 25.2                            & -                    & -                & 78.4                               & 90.3              &78.2   \\ \hline
% duck        & -                                 & -                                    & 19.6                                 & 17.2                                   & 19.2                                   & 15                                    & -                               & 65.6                            & -                    & -                 & 41.9                               & 77.7             & 52.1   \\ \hline
% eggbox      & -                                 & -                                    & 22                                   & 22.1                                   & 25.9                                   & 25.2                                  & -                               & 50.2                              & -                    & -                 & 80.9                               & 72.2             & 81.2    \\ \hline
% glue        & -                                 & -                                    & 38.5                                 & 35.8                                   & 39.6                                   & 32.4                                  & -                               & 49.6                              & -                    & -                & 68.1                               & 76.7              & 72.0   \\ \hline
% holepuncher & -                                 & -                                    & 22.1                                 & 36                                     & 21.3                                   & 49.5                                  & -                               & 39.7                              & -                    & -                 & 74.7                               & 91.4             & 75.2   \\ \hline \hline
% mean        & 6.4                               & 27.5                                   & 24.9                                 & 27                                     & 27                                     & 32                                    & 32.8                             & 40.8                              & 47.2                 & 58.4              & 63.2                               & 78               & 70.2    \\ \hline
% %   \end{tabularx}
% \end{tabular}
% \end{center}
% \\
% \caption{Occlusion LINEMOD Leaderboard}
% \label{tab:OccLinemod}
% %   } % \resizebox
% \end{table*}
% \end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[ht]
\begin{center}
%   \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\cline{3-11}
\multicolumn{2}{c|}{}
&
\multicolumn{7}{c}{Object} & \multirow{2}{*}{hole-}  
& %$\overline{\mbox{ADD(s)}}$ \\ % [3pt]
\\\cline{1-2}
%   \cline{11-11}
%   \hline
Descriptors      & ICP     & ape  & can  & cat  & driller & duck & eggbox$^{*}$ & glue$^{*}$ & puncher &
% \begin{tabular}{c}\vspace{-3 pt} 
% $\overline{\mbox{ADD(s)}} [\%]$ 
% \end{tabular}
Mean
\\\hline \hline
\multirow{2}{*}{PointNet++~\cite{qi2017pointnet++}}
& \xmark & 63   & 96.1 & 57.3 & 81.4  & 54.2 & 81.5  & 75.1 & 80.7 & 73.7\\ \cline{2-11}
& \checkmark & \textbf{65.7} & \textbf{96.4} & \textbf{58.5} & \textbf{81.7}  & \underline{54.7} & \textbf{82}    & \textbf{75.4} & 81.2 & \textbf{74.5}\\ \hline
\multirow{2}{*}{Point Transformer~\cite{zhao2021point}} & \xmark & 59.2 & 93.4 & 56.8 & 80.8 & 58.2 & 79.6 & 73.2 & 85.4 & 73.3 \\ \cline{2-11}
 & \checkmark & \underline{59.9}  & \underline{93.7} & \underline{57.2} & \underline{81.1} & \textbf{58.6} & \underline{80.1} & 73.6 & \underline{85.8} & \underline{73.8} \\ \hline
\multirow{2}{*}{PPF+knn} & \xmark & 55.7 & 88.6 & 51.2 &  78.2 & 54.1 & 79.4  & 73.8 & 85.7 & 70.8 \\\cline{2-11}
& \checkmark & 56.8 & 89.4 & 51.6 & 78.8 & 54.8 & 80.2  & \underline{74.3} & \textbf{87.2} & 71.7 \\\hline
\multirow{2}{*}{FPFH+knn} & \xmark & 55.4 & 89.2 & 50.2 & 77.8 & 52.6 & 80.9  & 72.4 & 86.3 & 70.6 \\\cline{2-11}
& \checkmark & 55.7 & 90.2 & 50.8 & 78.2  & 53.8 & 81.4 & 73.2 & \textbf{87.2} & 71.3 \\\hline
\multirow{2}{*}{DGCNN\cite{wang2019dgcnn}} & \xmark & 58 & 87.2 & 53.4 & 77.8  & 51.9 & 78.7  & 71.2 & 82.3 & 70.1\\\cline{2-11}
& \checkmark & 59.2 & 88.6 & 54.1 & 78.2  & 52.1 & 78.7  & 71.7 & 82.7 & 70.7 \\\hline
\multirow{2}{*}{SubdivNet\cite{hu2021subdivnet}} & \xmark & 42.3 & 83.2 & 49.2 &  77.8 & 48.7 & 77.9  & 69.2 & 75.2 & 65.4\\\cline{2-11}
& \checkmark & 45.2 & 83.7 & 49.7 & 78.2  & 49.2 & 78.2  & 70.1 & 75.2 & 66.2\\\hline

\end{tabular}
\end{adjustbox}
\end{center}
%   } % \resizebox
\caption{LMO accuracy results for different descriptors:
accuracy of RCVPose3D for non-symmetric objects is evaluated with ADD, and for
symmetric objects
(annotated with~$^{*}$) is evaluated with ADD-s.%  % RCVPose outperfoms for all the objects with an ICP refinement, specifically for small scale objects like ape, the performance boosted twice with ADD(s) metrics.
\label{tab:OccLinemodDescriptors}
}
 \vspace{-0.7\baselineskip}
\end{table*}

==> tabs/results_mean.tex <==
\begin{table}[t]
\begin{center}
%  \resizebox{\columnwidth}{!}{%
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|c|c|c}
\cline{4-6}
\multicolumn{3}{c|}{}

 & \multicolumn{2}{c|}{YCB} & LMO \\ \cline{3-6}
\multicolumn{2}{c|}{}&Optional

  &ADD(S) & ADD-S & $\mbox{ADD(s)}$\\ 
\cline{1-2}

Mode      & Method &Refine? &AUC &AUC& $ [\%]$
\\\hline \hline
                                & Oberweger~\cite{oberweger2018making} & \xmark  &72.8&-& 27.1\\\cline{2-6}  
                                & Hu et al.~\cite{hu2019segmentation}  &\xmark  &-&-& 30.4\\\cline{2-6}  
                                & Pix2Pose~\cite{park2019pix2pose} &  \xmark   &-&-& 32.0\\\cline{2-6}  
                                & \multirow{2}{*}{DPOD~\cite{zakharov2019dpod}}  &\xmark  &-&-& 32.8\\\cline{3-6}  
                                &  &\checkmark  &-&-& 47.3\\\cline{2-6}  
                                & PVNet~\cite{pvnet}    & \xmark   &73.4&-& 40.8\\\cline{2-6}  
%   \begin{rotate}{90} 

%   \end{rotate}
\multirow{-2}{*}{RGB}                                & PPRN~\cite{trabelsi2021ppn}  & \xmark   &83.1&-& 58.4\\\cline{2-6}  
%\multirow{-2}{*}{(D ref)}                                  & YOLO6D~\cite{yolo6d}  & \checkmark   &-&-& 6.4\\\cline{2-6}  
                                & SSD6D~\cite{kehl2017ssd}& \checkmark  &-&-& 27.5\\\cline{2-6}  
                               
    
                                &  \multirow{2}{*}{PoseCNN~\cite{posecnn}}   & \xmark  &59.9&75.8& 24.9\\\cline{3-6}
                              &  & \checkmark &85.4&93.0& - \\\cline{2-6} 
%   \begin{rotate}{90} 

%   \end{rotate}     
                                
                                 & GDR-Net~\cite{wang2021gdr} & \checkmark  &84.4&91.6& 62.2\\\cline{2-6} 
                                 & SO-Pose~\cite{Di_2021_ICCV} & \checkmark  &83.9&90.9& 62.3\\\hline\hline
& Tian et al.~\cite{tian2020robust}&\xmark  & - & 91.8  &-\\ \cline{2-6}  

                                & \multirow{2}{*}{RCVPose~\cite{wu2021vote}}      &  \xmark    & 95.2 & 96.6 & 70.2 \\\cline{3-6}  
%   \begin{rotate}{90} 
\multirow{+2.5}{*}{RGB-D/}  
%   \end{rotate}

& &\checkmark  & \underline{95.9} & \textbf{97.2}  & 71.1\\ \cline{2-6}  
\multirow{+2.5}{*}{RGB+3D}  & \multirow{2}{*}{PVN3D~\cite{pvn3d}} &\xmark   & 91.8 & 95.5 & 63.2\\\cline{3-6}
&  &\checkmark  & 92.3  & 96.1 & -\\\cline{2-6}
& FFB6D~\cite{he2021ffb6d}&\xmark  &92.7 &\underline{96.6} & 66.2\\\cline{2-6}  
& PointVoteNet\cite{hagelskjaer2020pointvotenet}   &\checkmark &-&-& \textbf{75.1}\\\hline\hline
\multirow{2}{*}{3D/Mesh}
& \multirow{2}{*}{BaseNet~\cite{gao20206d}}  &\xmark &- &91.4 & -\\ \cline{3-6}
&  &\checkmark &- & 94.7 & -\\ \cline{2-6}
& \multirow{2}{*}{RCVPose3D}  &\xmark &95.7 &96.3 & 73.7\\ \cline{3-6}
&  &\checkmark &\textbf{96.0} &\underline{96.6} & \underline{74.5}\\ \hline

\end{tabular}
\end{adjustbox}
\end{center}
%  } % \resizebox
\vspace{-1\baselineskip}
\caption{LMO and YCB average accuracy results.
%LMO is evaluated by ADD(S) and YCB is evaluated by ADD-S AUC and ADD(S) AUC %We are the second and only $0.6\%$ less than the RGB + point cloud method PointVoteNet. We outperformed all methods on YCB on the relatively strict metrics.
\label{tab:resultscombined}
}
\vspace{-1.5\baselineskip}
\end{table}
